Constraining parameters of low mass merging compact binary systems with Einstein Telescope alone

The Einstein Telescope (ET), a future third-generation gravitational wave detector will have detection sensitivity for gravitational wave signals down to 1 Hz. This improved low-frequency sensitivity of the ET will allow the observation of low mass binaries for a longer period of time in the detection band before their merger. Because of an improved sensitivity as compared to current and advanced 2G detectors, the detection rate will also be greatly improved. Given the high detection rate of merging compact binaries with the ET, it will be a useful instrument to conduct population studies. In this paper we present an algorithm to estimate the parameters of the low mass merging compact binary systems such as localization, chirp mass, redshift, mass ratios and total mass of the source which are crucial in order to estimate the capability of the ET to study various compact binary populations. For the compact binary population distributed uniformly in comoving volume we find that with single ET, $\approx 1\%$ of binaries can be localized within 800 square degrees. The values of chirp mass and total mass can be constrained within $\lesssim 5\%$ error, while $z$ and $D_L$ can be estimated with an error of $\lesssim 15\%$ for effective SNR $\gtrsim 50$ using single ET.

==> Constraining parameters of low mass merging compact binary systems with Einstein Telescope alone_arxiv/macros.tex <==
% macros.tex
%

% macro for 
\newcommand\note[1]{\textcolor{red}{\bf {#1}}}

%% Today macro \today
\renewcommand{\today}{\number\day\space\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\year}
\newcommand\checkme[1]{\textcolor{blue}{#1}}

\def\etc{{\it etc.}}
\def\eg{{\it e.g.}}
\def\vs{{\it vs.}}
\def\etal{{\it et al.}}
\def\ie{{\it i.e.}}
\def\cf{{\it cf.}}
\def\mycaps#1{{\textsc{\small #1}}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bi{\begin{itemize}} 
\def\ei{\end{itemize}}
\def\ben{\begin{enumerate}}
\def\een{\end{enumerate}}
%%\def\i{\item{}}      %--  \i is used to produce a dotless i, needed for Diaz
%\def\hrssu{\mathrm{strain}/\sqrt{\mathrm{Hz}}}
%\def\hrssu{strain/\sqrt{Hz}}
%\def\hrssu{Hz${}^{-1/2}$}
%\def\hrss{h_\mathrm{rss}}
%\def\hrssfifty{h_\mathrm{rss}^\mathrm{50\%}}
%\def\hdet{h_\mathrm{det}}
%\def\rninety{R_\mathrm{90\%}}
%\def\Zcoh{Z_{\text{H}_+}}
%\def\Zcor{Z^{corr}_{\text{H}_+}}
%\def\sfyo{S5y1}
%\def\sfyt{S5y2}
%\def\ligodoc{{LIGO-P17}{00177}{}} % leave in the extra {}s -- trust me

\def\aj{Astron. J.}
\def\apj{Astrophys. J.}
\def\apjl{Astrophys. J. Lett.}
\def\apjs{Astrophys. J. Supp. Ser. }
\def\aa{Astron. Astrophys. }
\def\aap{Astron. Astrophys. }
\def\araa{Ann.\ Rev. Astron. Astroph. }
\def\aapr{Astron. Astrophys. Rev. }
\def\physrep{Phys. Rep. }
\def\mnras{Mon. Not. Roy. Astron. Soc. }
\def\mmsun{M_\odot}
\def\prl{Phys. Rev. Lett.}
\def\prd{Phys. Rev. D.}
\def\azh{Soviet Astron.}
\def\apss{Astrophys. Space Sci.}
\def\cqg{Class. Quantum Grav.}
\def\memsai{Mem. Societa Astronomica Italiana}
\def\jcap{Journal of Cosmology and Astroparticle Physics}
\def\nat{Nature}
%\def{Science}
\def\bain{Bull. Astron. Inst. Netherlands}
\def\planss{Planet. Space Sci.,}
\def\ao{Appl. Opt.,}





